Toward computer-assisted discovery and automated proofs of cutting plane theorems

Using a metaprogramming technique and semialgebraic computations, we provide computer-based proofs for old and new cutting-plane theorems in Gomory--Johnson's model of cut generating functions.

==> Makefile <==
LATEX=latex
PDFLATEX=pdflatex
FIG2DEV=fig2dev
BIBTEX=bibtex

FIGURESDIRPREFIX=

MAINTEXFILE=param-abstract

all: $(MAINTEXFILE).pdf

%.pstex_t: %.fig #Makefile
	$(FIG2DEV) -L pstex_t -p $*.pstex $< $@

%.pstex: %.fig #Makefile
	$(FIG2DEV) -L pstex $< $@

%.pdftex_t: %.fig #Makefile
	$(FIG2DEV) -L pdftex_t -p $*.pdf $< $@

%.pdf: %.fig #Makefile
	$(FIG2DEV) -L pdftex $< $@

PARAM_GRAPHICS_SOURCES=

PARAM_GENERATED_GRAPHICS=$(PARAM_GRAPHICS_SOURCES:%.fig=$(FIGURESDIRPREFIX)%.pdftex_t) $(PARAM_GRAPHICS_SOURCES:%.fig=$(FIGURESDIRPREFIX)%.pdf) 

#$(PARAM_GRAPHICS_SOURCES:%.fig=%.pstex_t) $(PARAM_GRAPHICS_SOURCES:%.fig=%.pstex)

PARAM_SOURCES=Makefile $(MAINTEXFILE).tex $(PARAM_GRAPHICS_SOURCES:%.fig=$(FIGURESDIRPREFIX)%.fig) \
	sage-commands.tex									   \
	cpl_extreme_cases_diagrams.tex								   \
	param_3s_ext_1_f_diagrams.tex								   \
	param_3s_ext_2_f_diagrams.tex


PARAM_STYLES = llncs.cls

## copied these files from their source:
## $ (cd ~/Dropbox/yuan-group-relaxation-sage-code/ && tar cf - $files) | tar xvf -
PARAM_GRAPHICS=$(PARAM_GENERATED_GRAPHICS)					\
	param_graphics/plot_gj_forward_3_slope.pdf				\
	param_graphics/plot_drlm_backward_3_slope.pdf				\
	param_graphics/plot_chen_4_slope.pdf					\
	region_graphics/gj_forward_3_slope_claimed.pdf				\
	param_graphics/complex_gj_forward_3_slope_lambda_1_lambda_2_slice.png	\
	region_graphics/drlm_backward_3_slope_claimed.pdf			\
	param_graphics/flipineq_drlm_backward_3_slope_f_bkpt.png		\
	new_ext_graphics/plot_kzh_3_slope_param_extreme_1.png			\
	new_ext_graphics/plot_kzh_3_slope_param_extreme_2.png			\
	param_graphics/flipineq_gj_forward_3_slope_f_lambda_1.png		\
	param_graphics/flipineq_gj_forward_3_slope_f_lambda_2.png		\
	region_graphics/chen_4_slope_flawed_claimed.pdf				\
	param_graphics/flipineq_chen_4_slope_lam1_lam2.png			\
	cpl_graphics/regions87.png						\
	cpl_graphics/cpl_theta_1.png						\
	cpl_graphics/cpl_theta_2.png						\
	cpl_graphics/cpl_theta_3.png						\
	cpl_graphics/cpl_theta_4.png						\
	cpl_graphics/cpl_theta_5.png						\
	cpl_graphics/cpl_theta_6.png						\
	cpl_graphics/cpl_theta_7.png						\
	cpl_graphics/cpl_theta_8.png						\
	cpl_graphics/cpl_theta_9.png						\
	new_ext_graphics/param_3s_ext_1_f_1_over_19.png				\
	new_ext_graphics/param_3s_ext_1_f_6_over_19.png				\
	new_ext_graphics/param_3s_ext_1_f_2_over_19.png				\
	new_ext_graphics/param_3s_ext_1_f_7_over_19.png				\
	new_ext_graphics/param_3s_ext_1_f_3_over_19.png				\
	new_ext_graphics/param_3s_ext_1_f_8_over_19.png				\
	new_ext_graphics/param_3s_ext_1_f_4_over_19.png				\
	new_ext_graphics/param_3s_ext_1_f_9_over_19.png				\
	new_ext_graphics/param_3s_ext_1_f_5_over_19.png				\
	new_ext_graphics/param_3s_ext_1_f_10_over_19.png			\
	new_ext_graphics/param_3s_ext_2_f_3_over_9.png				\
	new_ext_graphics/param_3s_ext_2_f_6_over_9.png				\
	new_ext_graphics/param_3s_ext_2_f_4_over_9.png				\
	new_ext_graphics/param_3s_ext_2_f_7_over_9.png				\
	new_ext_graphics/param_3s_ext_2_f_5_over_9.png				\
	new_ext_graphics/param_3s_ext_2_f_8_over_9.png

copy-graphics-from-dropbox:
	(cd $$HOME/Dropbox/yuan-group-relaxation-sage-code/ && tar cf - $(PARAM_GRAPHICS)) | tar xvf -

BIB=../../bib/MLFCB_bib.bib

.PHONY: figures

figures: $(PARAM_GRAPHICS) 

$(MAINTEXFILE).pdf: $(MAINTEXFILE).tex $(PARAM_GRAPHICS) $(BIB)
	$(PDFLATEX) -halt-on-error "$<"
	$(BIBTEX) $(MAINTEXFILE)
	$(PDFLATEX) -halt-on-error "$<"
	$(PDFLATEX) -halt-on-error "$<"

PARAM_SOURCES_AND_MORE=$(PARAM_SOURCES) $(PARAM_GRAPHICS) $(PARAM_STYLES)

.PHONY: arxiv
arxiv:
	COPYFILE_DISABLE=true tar -cf $(CURDIR)/$(MAINTEXFILE).tar	\
		$(MAINTEXFILE).bbl					\
		$(PARAM_SOURCES)					\
		$(PARAM_GRAPHICS)					\
		$(PARAM_STYLES)
	rm -f $(MAINTEXFILE).tar.gz
	gzip $(MAINTEXFILE).tar

